Enhancing CLIP with CLIP: Exploring Pseudolabeling for Limited-Label Prompt Tuning

Fine-tuning vision-language models (VLMs) like CLIP to downstream tasks is often necessary to optimize their performance. However, a major obstacle is the limited availability of labeled data. We study the use of pseudolabels, i.e., heuristic labels for unlabeled data, to enhance CLIP via prompt tuning. Conventional pseudolabeling trains a model on labeled data and then generates labels for unlabeled data. VLMs' zero-shot capabilities enable a "second generation" of pseudolabeling approaches that do not require task-specific training on labeled data. By using zero-shot pseudolabels as a source of supervision, we observe that learning paradigms such as semi-supervised, transductive zero-shot, and unsupervised learning can all be seen as optimizing the same loss function. This unified view enables the development of versatile training strategies that are applicable across learning paradigms. We investigate them on image classification tasks where CLIP exhibits limitations, by varying prompt modalities, e.g., textual or visual prompts, and learning paradigms. We find that (1) unexplored prompt tuning strategies that iteratively refine pseudolabels consistently improve CLIP accuracy, by 19.5 points in semi-supervised learning, by 28.4 points in transductive zero-shot learning, and by 15.2 points in unsupervised learning, and (2) unlike conventional semi-supervised pseudolabeling, which exacerbates model biases toward classes with higher-quality pseudolabels, prompt tuning leads to a more equitable distribution of per-class accuracy. The code to reproduce the experiments is at https://github.com/BatsResearch/menghini-neurips23-code.

==> sections/old_material.tex <==
%CLIP (citation) is a VLM which consists of a separate text encoder $\psi$ and an image encoder $\phi$, jointly trained on XXX million image-text pairs. The encoders were trained using a contrastive loss, which aimed to maximize the cosine similarity of matching image-text pairs, and minimize the cosine similarity of image-text pairs that do not match. In this way, the common projection space $\mathbb{R}^d$ is "aligned" in its representations of images and text. 

%CLIP comes with multiple image encoders of varying sizes. Some use a modified ResNet-50 (citation) architecture, and others use a vision transformer architecture (ViT) (citation). 
%CLIP's structure enables zero-shot image classification. 
% Given $n$ target classes $Y = \{y_1, ..., y_n\}$, we define $n$ textual prompts, such as $p_i = $"a photo of a [CLASS$_i$]", where CLASS$_i$ is replaced by the specific class name, such as “dog,” “forest” or “Boeing 737.”. These handcrafted prompts are used to generate weight vectors in the shared embedding space via the text encoder, such that $w_i = \psi(p_i)$. Finally, these weight vectors, along with the image features $z = \phi(x)$ are used for classification according to:
% \begin{align*}
%     p(y=i \mid \boldsymbol{x})= \frac{\exp \left(\cos \left(\boldsymbol{w}_i, \boldsymbol{z}\right) / \tau\right)}{\sum_{j=1}^k \exp \left(\cos \left(\boldsymbol{w}_j, \boldsymbol{z}\right) / \tau\right)}
% \end{align*}
% where cos(·, ·) denotes the cosine similarity and $\tau$ is a fixed temperature value.
% % NOTE: UPT has this below section which I think makes sense/could be helpful for the reader. I could consider adding something like this


% Conceptually, such a decision process for the input image x in Eq. (1) is formulated in a way that the text encoder takes a role of generating dynamic classifiers W from open-set categories Y, with the image encoder producing encoded visual features z.


% Before the era of VLMs, generating pseudolabels required access to at least some labeled data to train a primer task-specific classifier.
% This limited the use of pseudolabeling to the semi-supervised learning setting, where a small amount of labeled data was available.
% However, with VLMs, pseudolabels can be generated regardless of the data availability setting, and open up a wide range of applications for the technique.





% The widespread adoption of VLMs has greatly expanded the applications of pseudolabeling as a technique for leveraging unlabeled data. With their powerful general-purpose classification abilities, VLMs can generate high-quality pseudolabels, which can be used to train classifiers on larger and more diverse datasets.

% Before the era of VLMs, generating pseudolabels required access to at least some labeled data to train a primer task-specific classifier. This limited the use of pseudolabeling to the semi-supervised learning setting, where a small amount of labeled data was available. However, with VLMs, pseudolabels can be generated regardless of the learning setting, enabling their application in both supervised and unsupervised learning.

% Overall, the availability of pseudolabeling as a technique for leveraging unlabeled data, thanks to the advancements in VLMs, opens up new avenues for data-driven applications and can lead to significant improvements in the performance of machine learning models.

% This makes pseudolabeling a powerful tool for both supervised and unsupervised learning, and has greatly expanded the range of applications for the technique.


% Unlabeled data generally complements or substitutes scarce labeled data and is leveraged through unsupervised losses or pseudolabeling.
% While pseudolabeling is typically associated with semi-supervised learning, where a small number of labeled instances are needed to first train a classifier that generates target-related pseudolabels for the unlabeled data, the emergence of general-purpose zero-shot classifiers eliminates the need for a separate classifier to generate pseudolabels. 
% This development enables VLMs to seamlessly leverage unlabeled data, making pseudolabeling a natural way to adapt them to new tasks beyond just semi-supervised learning settings.
% While unsupervised losses are commonly used in various data availability settings, pseudolabels are typically associated with semi-supervised learning, where a small number of labeled instances are needed to first train a classifier that generates target-related pseudolabels for the unlabeled data.
% However, in the era of general-purpose zero-shot classifiers, the need for training a classifier to generate pseudolabels is no longer necessary. 
% Instead, pseudolabeling becomes a natural way of leveraging unlabeled data, relying on the resourceful knowledge of VLMs and their zero-shot transfer capabilities, and opens up the possibility of VLM adaptation through pseudolabels in settings beyond just semi-supervised learning. 

% In the era of general-purpose zero-shot classifiers, the need for the last passage is no longer necessary, as these classifiers can be utilized as general-purpose pseudolabelers. By combining the resourceful knowledge of VLMs and their zero-shot transfer capabilities, pseudolabeling becomes a natural way to leverage unlabeled data, opening up the possibility of pursuing VLM adaptation through pseudolabels in settings beyond just semi-supervised learning.




% Instead, the resourceful knowledge of VLMs and their zero-shot transfer capabilities can be combined to leverage unlabeled data, and enable VLM adaptation through pseudolabels in settings beyond just semi-supervised learning. 
% Our results demonstrate the effectiveness of our proposed approach, highlighting the potential of VLM adaptation through pseudolabels in real-world applications.
% nell'era di zsl this last passage no longer required - thus combinig the power of VLM with their being zsl, pseudolabels are a natural way of augmenting training dataset opening the possibility of pursuing the route of VLM adaptation relying on pseudolabels for a wide range of learning settings.
% For this reason, exploiting unlabeled data by using pseudlabels has been limited to semi-supervised learning scenario.
% On the contrary, in the era of general-purpose zero-shot classifiers, pseudolabeling is a natural route to adapt VLMs relying on 
% 2. Pseudolabeling natural but under explored route for adaptation  //  — surprisingly not used that much
% Generalization beyond semi-supervised learning, lots of thing with pseudolabelings
% Large pre-trained vision-language models (VLMs) achieve remarkable levels of accuracy without the need for task-specific training. 
% However, in more specialized domains, they tend to underperform and require additional adaptation for optimal performance. 
% This reignites a long-standing bottleneck in machine learning: the lack of labeled data. 
% Before the emergence of VLMs, the challenge of learning with limited labeled data has been extensively studied and diverse approaches were taken to address different data availability settings. 
% In this paper, we explore the feasibility of defining a unified learning framework to adapt VLMs with limited labeled data. 
% Our goal is to investigate training strategies that can be applied seamlessly across various data availability settings, 


% Large pre-trained vision-language models (VLMs), such as CLIP~\citep{Radford2021LearningTV}, ALIGN~\citep{Jia2021ScalingUV}, and Florence~\citep{Yuan2021FlorenceAN}, have significantly advanced the field of image classification by achieving exceptional levels of accuracy without requiring task-specific training. 
% However, they tend to underperform in more specialized domains, such as satellite image classification and fine-grained tasks like identifying flower species or textures~\citep{Radford2021LearningTV}. 
% \emph{Prompt-tuning} has emerged as an efficient and effective solution to improve VLMs performance by fine-tuning the model's inputs using a few labeled instances per target class~\citep{lester-etal-2021-power,Zhou2021LearningTP}.
% While this approach has shown promise in adapting VLMs to specialized domains, a major overlooked challenge is how to achieve similar improvements when labeled data is limited or unavailable, and unlabeled data is abundant. 
% Thus, a question raises: \emph{how can we utilize unlabeled data in prompt-tuning to effectively enhance the performance of VLMs? What advantages can this approach offer?}


% The scarcity of data in specialized domains can pose significant challenges to achieving satisfactory performance with VLMs. 
% This limitation can impede the fine-tuning of prompts that effectively adapt to new domains, potentially hindering the adoption of VLMs and limiting their potential benefits.
% When abundant unlabeled target data is available, the VLM's zero-shot transfer capabilities can be utilized to generate pseudolabels.

%%% Abstract
% In contrast to earlier methods of generating pseudolabels, which depended on labeled data for their creation and were mostly applied in semi-supervised learning settings, utilizing vision-language models such as CLIP as general-purpose pseudolabelers offers a more versatile approach for learning from unlabeled data in any scenario with limited labeled data.
    % Standard methods of generating pseudolabels rely on labeled data for their creation and are mostly applicable in semi-supervised learning settings. In contrast, utilizing vision-language models, such as CLIP, as general-purpose pseudolabelers offers a more versatile approach for learning from unlabeled data in any scenario with limited labeled data.
    % \cri{should we enumerate what case the study covers? Like different prompt tuning modalities, learning paradigms?}
    % Our research demonstrates that second-generation pseudolabeling facilitates the development of versatile training strategies that can be applied in various settings.
    % which indicates that they can be effectively addressed using similar approaches.
    % Additionally, 
    % prompts learned via iterative strategies determine a significantly more equitable distribution of accuracy across classes.

    % tuning prompts for CLIP positively impact its prediction distribution of CLIP no longer biased toward by showing a .
        % Being the adaptation of CLIP largely unexplored in settings with limited labeled data, a part for few-shot learning, we run a comprehensive analysis of prompt-tuning techniques under diverse learning settings 
    % This approach not only effectively adapts CLIP to target tasks and enhances training efficiency
    % Vision-language models can function as general-purpose pseudolabelers to enable learning from unlabeled data in scenarios with limited labeled data.
    % This approach differs from previous use of pseudolabels, which required access to labeled data for their generation, thereby limiting their applicability to only semi-supervised learning settings.
    % This is opposed to previous usage of pseudolabels whose generation required access to labeled data, limiting its usage only to semi-supervised learning settings.
        % \item CLIP for CLIP: Can we Define a Unified Learning Framework for Prompt Tuning with Limited Labeled Data?
        % \item CLIP for CLIP: Prompt Tuning with Pseudolabels to Unify Learning with Limited Labeled Data
        % \item CLIP for CLIP: Towards a Unified Learning Framework for Prompt Tuning with Limited Labeled Data

  
    % In a set of image classification tasks where CLIP exhibits limitations, we demonstrate that unexplored training strategies that iteratively refine pseudolabels are effective methods to learn task-related prompts. 
    % This results in consistent improvements over CLIP, as well as standard prompt-tuning strategies, in semi-supervised, transductive zero-shot, and unsupervised learning.
    % In addition, as opposed to earlier semi-supervised methods using pseudolabeled data, which exacerbate model's biases toward certain classes, using iterative strategies to learn prompts results in a more equitable distribution of accuracy across all classes.


%%%% ABSTRACT.2
    % Standard pseudolabeling involves training a model on labeled data, and then use it to generate labels for unlabeled data. Vision-language models (VLMs) such as CLIP have given rise to a ``second generation'' of pseudolabeling, that eliminates the need for labeled data. By leveraging their zero-shot capabilities, VLMs can generate labels without additional training. This expands the scope of pseudolabeling beyond its traditional application in semi-supervised learning, making it a valuable technique for a wider range of scenarios with limited labeled data. In this paper, we study how to use CLIP's self-produced pseudolabels to improve  CLIP itself via prompt tuning, when labeled data is scarce. Relying on second-generation pseudolabeling, we observe that learning paradigms such as semi-supervised, transductive zero-shot, and unsupervised learning, can be seen as special cases of a unified learning loss, enabling the development of versatile training strategies applicable in various settings. We investigate the effectiveness of multiple training strategies image classification tasks where CLIP exhibits limitations, by varying prompt modalities and learning paradigms. We investigate the effectiveness of multiple training strategies on a set of image classification tasks where the CLIP exhibits limitations, by varying prompt modalities and learning paradigms. We found that (1) unexplored strategies that iteratively refine pseudolabels consistently improve CLIP, by X in semi-supervised learning, by Y in transductive zero-shot learning, and by Z in unsueprvised learning; (2) interestingly, we observed that these improvements occurred regardless of prompt modality, although textual prompts appeared to be more effective, (3) unlike earlier semi-supervised methods that rely on pseudolabeled data, which may exacerbate model biases toward certain classes, iterative strategies learn prompts resulting in a more equitable distribution of CLIP's accuracy across all classes.



    % Standard pseudolabeling involves training a model on labeled data, and then use it to generate labels for unlabeled data.  The zero-shot capabilities of vision-language models (VLMs) like CLIP have sparked a promising ``second generation'' of pseudolabeling that eliminates the need for labeled data to generate labels. This expands pseudolabeling's scope  beyond semi-supervised learning, making it a valuable technique for a broader range of scenarios with limited labeled data. In this paper, we study how to use CLIP's self-produced pseudolabels to improve CLIP itself on downstream tasks via prompt tuning.
    
    % Improving the ability to adapt vision-language models (VLMs) like CLIP to downstream tasks with limited labeled data is crucial for scaling the practical usage of these models.
    % The zero-shot capabilities of VLMs have sparked a promising ``second generation'' of pseudolabeling that eliminates the need for labeled data to generate labels, in contranst to standard pseudolabeling that involves training a model on labeled data, and then use it to generate labels for unlabeled data.
    % This expands pseudolabeling's scope beyond semi-supervised learning, making it a valuable technique for a broader range of scenarios with limited labeled data.

    % Enhancing vision-language models (VLMs) like CLIP on downstream tasks with limited labeled data is a crucial but underexplored problem for scaling the practical usage of these models.
    % The zero-shot capabilities of CLIP unlock a ``second generation'' of pseudolabeling approaches that eliminate the need for labeled data to generate labels, and expand pseudolabeling's scope beyond traditional semi-supervised learning, making it a valuable technique for a broader range of scenarios with limited labeled data.
    % When unlabeled data substitutes or complements labeled data, how do we improve the performance of vision-language models (VLMs) like CLIP on target tasks?
    % Improving the performance of vision-language models (VLMs) like CLIP on downstream tasks with limited labeled data is an underexplored problem. 
    % In the presence of unlabeled data, one can exploit VLMs' zero-shot capabilities and generate pseudolabels for training. 
    % In this paper, we study how to use CLIP's self-produced pseudolabels to improve  
    % CLIP itself on downstream tasks via prompt tuning.
    % Standard pseudolabeling involves training a model on labeled data, and then use it to generate labels for unlabeled data. 
    % VLMs' zero-shot capabilities enable a "second generation" of pseudolabeling approaches that do not require labeled data to generate labels. 
    % This expands pseudolabeling's scope beyond semi-supervised learning, making it a valuable technique for a broader range of scenarios with limited labeled data.

    % This  ``second generation'' of pseudolabeling, which eliminates the need of labeled data to generate labels, expands pseudolabeling's scope beyond semi-supervised learning, making it a valuable technique for a broader range of scenarios with limited labeled data.
    % VLMs have zero-shot capabilities, which give rise to a ``second generation'' of pseudolabeling that eliminates the need of labeled data to generate labels, unlike standard pseudolabeling that relies on training a model on labeled data. 
    % This expands pseudolabeling's scope beyond semi-supervised learning, making it a valuable technique for a broader range of scenarios with limited labeled data.
    % Say that 
    % , when labeled data is scarce.    
    % Standard pseudolabeling involves training a model on labeled data, and then use it to generate labels for unlabeled data.
    % Standard pseudolabeling involves training a model on labeled data, and then use it to generate labels for unlabeled data.
    % The zero-shot capabilities of CLIP spark a promising ``second generation'' of pseudolabeling that eliminates the need for labeled data to generate labels.
    % This expands pseudolabeling's scope beyond semi-supervised learning, making it a valuable technique for a broader range of scenarios with limited labeled data.
    % The zero-shot capabilities of VLMs give rise to a ``second generation'' of pseudolabeling, which eliminates the need of labeled data to generate labels, unlike standard pseudolabeling that needs labeled data for training. This expands the usefulness of  pseudolabeling's scope beyond semi-supervised learning, making it valuable for a broader range of scenarios with limited labeled data.
    % Using second-generation pseudolabeling, we observe that learning paradigms like semi-supervised, transductive zero-shot, and unsupervised learning unify under a single loss, enabling the development of versatile training strategies that are applicable in various settings.
    % We investigate multiple training strategies on image classification tasks where CLIP exhibits limitations, by varying prompt modalities, e.g., textual or visual prompts, and learning paradigms.
    % We found that (1) unexplored strategies that iteratively refine pseudolabels consistently improve CLIP, by X in semi-supervised learning, by Y in transductive zero-shot learning, and by Z in unsupervised learning;
    % (2) CLIP improvements occur regardless of the prompt modality, although textual prompts are more effective, 
    % (3) unlike earlier usage of pseudolabeled data, which exacerbates model biases toward certain classes, we note a more equitable distribution of accuracy across all classes.





    % Standard pseudolabeling relies on labeled data and is mainly suitable for semi-supervised learning.~\cri{Maybe I want to simply explain how it used to be before CLIP. This can be criptic.} 
    % In contrast, using vision-language models like CLIP as general purpose pseudolabelers~\cri{Is it clear that this is because of zero-shot transfer abilities of VLMs} offers the possibility of learning from unlabeled data in any scenario with limited labeled data.
    
    % First generation: labeled data to learn a primer task-specific classifier, then produce pseudolabels - application limited to semi-supervised settings
    % Second generation: labeled data no longer a requirement, vlms spits out labels without further tuning on the target task.
    % This expands the applicability of pseudolabels to wider range of settings.
    % Say that we study such training strategies varying the prompts modalities and learning paradigms on a set of image classification tasks where CLIP shows limits
    % We observe that (1) simple iterative consistent improvements across learning strategies (2) consistent behaviour across prompt modalities, all improve but textual prompts are superior (3) as opposed to earlier use of pseudolabels which exacerbate model's biases toward certain classes, the learned prompts results in a equitable distribution of CLIP's accuracies across all target classes.
    % SHORTER VERSION

%%%%% Intro

% In this study, we explore \name{} by comprehensively analyzing the effectiveness of utilizing pseudolabels for \pinkbox{prompt-tuning} across various \greenbox{learning paradigms} and \bluebox{training strategies}. 
% Our main focus is to validate underexplored training strategies that utilize pseudolabels, with the ultimate goal of enhancing VLMs' performance on target tasks that exhibit a significant domain gap from their pre-training dataset.
% Additionally, we explore VLM predictions using \shortname{} under different settings, to gain a qualitative understanding of what these models learn from pseudolabels. By scrutinizing these predictions, we hope to unravel the inner workings of \shortname{} and unlock new insights into its capabilities, paving the way for more effective and efficient learning strategies.
% \Cref{fig:overview} shows an overview of the settings we consider to provide guidelines on the recommended usage, benefits, and limitations of \shortname. 



%  INTRO

% Previously, generating pseudolabels for unlabeled data required access to at least some labeled data to train a task-specific classifier, and it was associated to semi-supervised learning~\citep{Lee2013PseudoLabelT,NEURIPS2021_995693c1,NEURIPS2019_1cd138d0}. 
% Instead, VLMs can produce pseudolabels out-of-the-box, eliminating the need labeled data and opening up a vast range of possible applications.
% VLMs can now generate pseudolabels regardless of the availability of labeled data, opening up a vast range of possible applications.
% In this paper, we revisit pseudolabeling in the era of large pre-trained models and thoroughly explore how they contribute to developing general purpose training strategies applicable across diverse data availability scenarios.

% Learning with limited labeled data includes paradigms such as semi-supervised learning, transductive zero-shot learning, and unsupervised learning. 
% These paradigms leverage unlabeled data to complement or substitute scarce labeled data, and its optimal use depends on the specific setting and requires careful consideration. 
% In the context of VLMs, prompt-tuning has emerged as an efficient and effective solution for improving performance by fine-tuning the model's inputs using a few labeled instances per target class. 
% However, applying prompt-tuning in different data availability settings requires tailored training strategies. 

% As we seek to enhance CLIP's performance in specialized domains, the use of CLIP-generated pseudolabels presents a potential solution. 
% However, relying on pseudolabels when CLIP may not perform optimally in these domains also carries inherent risks. 
% \emph{How can we effectively leverage pseudolabels without compromising performance or introducing errors?}



% Say a few words about pseudolabels and intutition behind. It's empiric, effect can vary depending on the accuracy of pseudolabels combined to the usage we make of it.
% Since we focus on investigating how to use CLIP for CLIP, thus how to improve CLIP accuracy via prompts we consider three dimension for our study
% the space of prompting - what we train, learning paradigms - what data we have, and training strategies - how we use pseudolabels.
% Highlight the importance of of having accurate and unbiased pseudolabels
% Mention the challenges of pseudolabeling with CLIP: biased predictions, accuracy varies across classes


% However, applying prompt-tuning in different data availability settings requires tailored training strategies. While this may seem to go against the goal of developing large pre-trained models that can be applied effortlessly to various problems, it is necessary to achieve optimal performance. 
% To reconcile the need for specificity with the need for generalization, we explore modular training strategies that can be distilled into a single learning objective. 
% This approach can enable easy customization to different availability settings, reducing the need for proposing numerous and diverse approaches while still achieving VLMs’ performance improvement across a range of learning paradigms.


% With training strategies unified across both prompt modalities and learning settings, we can expreiment different usage of pseudolabels for any combination of prompts modalities, learning paradigms, and learning strategies depicted in Figure 1.
% To our best knowledge, among all the possible paths, only one has been explored. Huang et al. investigated how to fine-tune prompts in an unsupervised learning setting using few-pseudolabels.
% We go well-beyond the only unsupervised setting and instead of relying on a fixed set of unlabeled data, we investigate iterative training approaches that enable ongoing refinement and expansion of the pool of pseudolabeled data employed during training, namely IFPL and GRIP in Figure 1. 


% Similarly to [CITE], we treat unlabeled data as labeled data and fine-tune prompts by optimizing a cross-entropy loss.  
% The use of pseudolabels for prompt tuning was introduced for unsupervised learning and proved to be effective to improve CLIP when only unlabeled data was available [CITE]. 
% However, [CITE] did not expand their study to other data settings and, along the lines of previous prompt-tuning works, they consider a unique training strategy that uses a small number of pseudolabeled instances per target class. 

% we observe good improvemtexamine the effectiveness of using a limited number of labeled samples for prompt fine-tuning, and find that iterative approaches that gradually incorporate all available unlabeled data are more successful, as they can mitigate the errors introduced by CLIP-generated  pseudolabels. 



% With training strategies unified across both prompt modalities and learning settings, we can expreriment different usage of pseudolabels for any combination of prompts modalities, learning paradigms, and learning strategies depicted in Figure 1.
% To our best knowledge, among all the possible paths, only one has been explored. Huang et al. investigated how to fine-tune prompts in an unsupervised learning setting using few-pseudolabels.
% We go well-beyond the only unsupervised setting, exploring also semi-supervised, and transductive zero-shot learning, and instead of relying on a fixed set of unlabeled data, we investigate iterative training approaches that enable ongoing refinement and expansion of the pool of pseudolabeled data employed during training, namely IFPL and GRIP in Figure 1. 


% We showcase that prompt tuning vision-language models with limited labeled data can be integrated into a unified framework, by leveraging self-produced pseudolabels. 
    % This unified framework simplifies the learning process across diverse data availability scenarios. 
    % Through a single objective function that utilizes pseudolabeled data as an entropy regularizer, different learning paradigms can be considered as special cases, allowing for the definition of data availability agnostic training strategies and reducing the requirement for numerous specialized approaches.


% Within this manuscript, our aim is to delve into the realm of utilizing preassigned pseudolabels, generated by the CLIP system, in order to enhance the overall performance of CLIP. 
% Consequently, we embark upon an extensive exploration encompassing a diverse range of prompt learning scenarios, wherein we manipulate prompt modalities, learning paradigms, and training strategies. 
% Remarkably, we present compelling empirical evidence demonstrating the noteworthy effectiveness of prompt training strategies that leverage CLIP-derived pseudolabels, irrespective of learning paradigms and prompt modalities, thereby leading to significant enhancements in CLIP's performance across various contexts.


% This paper investigates how the use of out-of-the-box pseudolabels assigned by CLIP can contribute to improving CLIP's own performance. 
% To achieve this, we explore a wide range of learning scenarios by varying prompt modalities, learning paradigms, and training strategies. 
% We present the initial evidence showcasing the effectiveness of prompt training strategies that utilize CLIP-based pseudolabels, regardless of learning paradigms and prompt modalities, resulting in notable improvements in CLIP's performance across different settings.




% \begin{table*}[ht]
%     \centering
%      \resizebox{\linewidth}{!}{
%     \begin{tabular}{lccccccccccccccccccc}
%     \toprule
%     % \multicolumn{2}{c}{Grocery Store Dataset}
%        & \multicolumn{3}{c}{Flowers102} & \multicolumn{3}{c}{RESICS45} & \multicolumn{3}{c}{FGVCAircraft} & \multicolumn{3}{c}{MNIST} & \multicolumn{3}{c}{EuroSAT} & \multicolumn{3}{c}{DTD}\\
%      \midrule
%      Method  & Text & Image & Multi & Text & Image & Multi & Text & Image & Multi & Text & Image & Multi & Text & Image & Multi & Text & Image & Multi\\
%      \cmidrule(lr){1-1} \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} \cmidrule(lr){14-16} \cmidrule(lr){17-19} %\cmidrule(lr){20-22}
%      CLIP & \multicolumn{3}{c}{$63.67_{0.00}$} & \multicolumn{3}{c}{$54.48_{0.00}$} & \multicolumn{3}{c}{$17.58_{0.00}$} & \multicolumn{3}{c}{$25.10_{0.00}$} & \multicolumn{3}{c}{$32.88_{0.00}$} & \multicolumn{3}{c}{$43.24_{0.00}$} \\
%      Base & $76.76_{1.11}$ & $63.73_{1.52}$ & $68.03_{1.29}$ & $58.53_{10.80}$ & $60.8_{1.64}$ & $62.84_{1.05}$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $37.1_{5.45}$ & $36.41_{2.17}$ & $43.71_{2.18}$ \\
%      FPL & $75.96_{0.74}$ & $67.03_{0.64}$ & $72.54_{0.35}$ & $68.13_{0.54}$ & $65.14_{0.24}$ & $66.96_{0.48}$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $50.77_{0.71}$ & $47.6_{1.09}$ & $48.32_{0.66}$ \\
%      IFPL & $78.68_{0.75}$ & $\mathbf{68.69_{0.44}}$ & $-$ & $70.52_{1.11}$ & $67.11_{1.18}$ & - & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $\mathbf{55.24_{0.96}}$ & $51.65_{0.69}$ & $-$ \\
%      GRIP & $\mathbf{83.6_{0.48}}$ & $67.95_{1.02}$ & - & $\mathbf{74.11_{0.68}}$ & $\mathbf{71.22_{0.77}}$ & - & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $\mathbf{56.07_{0.85}}$ & - & - \\
%      \midrule
%      $\Delta$ CLIP & + 19.93 & + 5.02 & - & + 19.53 & + 16.64 & - & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & + 12.83 & - & - \\
%      $\Delta$ Base & + 6.84 & + 4.96 & - & + 15.58 & + 10.42 & - & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & + 18.97 & - & - \\
%     \bottomrule
%     \end{tabular}}
%     \caption{\textbf{Semi-supervised learning}: Accuracy on FRAMED using CLIP ViT-B/32. The $\Delta$s are computed with respect to the max accuracy between IFPL and GRIP.}
% \label{tab:acc:gs_and_fms}
% \end{table*}


% \Cref{fig:quantity_vs_quality} shows the quality of pseudolabels throughout the iterative learning processes of textual prompts.

% \cref{fig:quantity_vs_quality} illustrates the quality of pseudolabels throughout the iterative learning process of textual prompts.

% In the IFPL approach, the number of pseudolabels remains fixed at 16, with refinement occurring at each iteration. 
% This consistent refinement process leads to a notable improvement in pseudolabel quality by the end of the process.


% For IFPL, the number of pseudolabels is fixed at 16, and they are refined with each iteration. 
% This process consistently improves the quality of the pseudolabels by the end of the process.




% Indeed, if we compare the quality of the expanded set of pseudodabels using GRIP and CLIP, we see that GRIP pseudolabels are of better quality than CLIP.
% Interestingly, even when the accuracy of IFPL pseudolabels is higher than that of GRIP at the last iteration, we see that the performance of GRIP is better. 
% This seems to be a pay-off of the larger number of pseudolabels on which GRIP is trained.
% Here we highlight that very good pseudolabels can limit the performance of the model against bit noisier pseudolabels which are instead numerous. 
% We highlight how this observation can be insightful for further development of approaches that might exploit this trade-off.


% \begin{figure}[htbp]
%   \centering
%   \begin{subfigure}{.15\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{images/bias/Flowers102_SSL_textual_fpl.pdf}
%     % \caption{F - FPL}
%     \label{fig:plot1}
%   \end{subfigure}
%   \hfill
%   \hspace{-5em}
%   \begin{subfigure}{.15\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{images/bias/Flowers102_SSL_textual_ifpl.pdf}
%     % \caption{F - IPFL}
%     \label{fig:plot1}
%   \end{subfigure}
%   \hfill
%   \hspace{-5em}
%   \begin{subfigure}{.15\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{images/bias/Flowers102_SSL_textual_grip.pdf}
%     % \caption{F - GRIP}
%     \label{fig:plot1}
%   \end{subfigure}
%   \hfill
%   \hspace{-5em}
%   \begin{subfigure}{.15\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{images/bias/DTD_SSL_textual_fpl.pdf}
%     % \caption{D - FPL}
%     \label{fig:plot1}
%   \end{subfigure}
%   \hfill
%   \hspace{-5em}
%   \begin{subfigure}{.15\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{images/bias/DTD_SSL_textual_ifpl.pdf}
%     % \caption{D - IFPL}
%     \label{fig:plot1}
%   \end{subfigure}
%   \hfill
%   \hspace{-5em}
%   \begin{subfigure}{.15\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{images/bias/DTD_SSL_textual_grip.pdf}
%     % \caption{D - GRIP}
%     \label{fig:plot1}
%   \end{subfigure}
%   \\
%   \vspace{-1.95em}
%   \begin{subfigure}{.15\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{images/bias/Flowers102_UL_textual_fpl.pdf}
%     % \caption{F - FPL}
%     \label{fig:plot1}
%   \end{subfigure}
%   \hfill
%   \hspace{-5em}
%   \begin{subfigure}{.15\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{images/bias/Flowers102_UL_textual_ifpl.pdf}
%     % \caption{F - IFPL}
%     \label{fig:plot1}
%   \end{subfigure}
%   \hfill
%   \hspace{-5em}
%   \begin{subfigure}{.15\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{images/bias/Flowers102_UL_textual_grip.pdf}
%     % \caption{F - GRIP}
%     \label{fig:plot1}
%   \end{subfigure}
%   \hfill
%   \hspace{-5em}
%   \begin{subfigure}{.15\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{images/bias/DTD_UL_textual_fpl.pdf}
%     % \caption{D - FPL}
%     \label{fig:plot1}
%   \end{subfigure}
%   \hfill
%   \hspace{-5em}
%   \begin{subfigure}{.15\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{images/bias/DTD_UL_textual_ifpl.pdf}
%     % \caption{D - IFPL}
%     \label{fig:plot1}
%   \end{subfigure}
%   \hfill
%   \hspace{-5em}
%   \begin{subfigure}{.15\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{images/bias/DTD_UL_textual_grip.pdf}
%     % \caption{D - GRIP}
%     \label{fig:plot1}
%   \end{subfigure}
%   \\
%   \vspace{-1.95em}
%   \begin{subfigure}{.15\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{images/bias/Flowers102_TRZSL_textual_fpl.pdf}
%     \caption{F - FPL}
%     \label{fig:plot1}
%   \end{subfigure}
%   \hfill
%   \hspace{-5em}
%   \begin{subfigure}{.15\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{images/bias/Flowers102_TRZSL_textual_ifpl.pdf}
%     \caption{F - IFPL}
%     \label{fig:plot1}
%   \end{subfigure}
%   \hfill
%   \hspace{-5em}
%   \begin{subfigure}{.15\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{images/bias/Flowers102_TRZSL_textual_grip.pdf}
%     \caption{F - FPL}
%     \label{fig:plot1}
%   \end{subfigure}
%   \hfill
%   \hspace{-5em}
%   \begin{subfigure}{.15\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{images/bias/DTD_TRZSL_textual_fpl.pdf}
%     \caption{D - FPL}
%     \label{fig:plot1}
%   \end{subfigure}
%   \hfill
%   \hspace{-5em}
%   \begin{subfigure}{.15\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{images/bias/DTD_TRZSL_textual_ifpl.pdf}
%     \caption{D - IFPL}
%     \label{fig:plot1}
%   \end{subfigure}
%   \hfill
%   \hspace{-5em}
%   \begin{subfigure}{.15\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{images/bias/DTD_TRZSL_textual_grip.pdf}
%     \caption{D - GRIP}
%     \label{fig:plot1}
%   \end{subfigure}
%   \caption{Comparison of the accuracy of pseudolabels during training.}
%   \label{fig:quantity_vs_quality}
% \end{figure}



% Pseudolabeled data can be obtained in multiple ways and each influences the quality of the final model's predictions~\citep{Xu2021DashSL,NEURIPS2021_995693c1,Iscen2019LabelPF,Shi2018TransductiveSD}.
% Some approaches use pseudolabels obtained on all unlabeled data~\citep{Lee2013PseudoLabelT} or average predictions from multiple augmentations as pseudolabels~\citep{NEURIPS2019_1cd138d0}. Others adopt confidence

% thresholds to generate pseudolabels on weakly augmented samples and utilize these pseudolabels as annotations for strongly augmented samples~\citep{sohn20Fixmatch,Berthelot2020ReMixMatch:,NEURIPS2020_44feb009}. 

